Robust Probabilistic Model Checking with Continuous Reward Domains

Probabilistic model checking traditionally verifies properties on the expected value of a measure of interest. This restriction may fail to capture the quality of service of a significant proportion of a system's runs, especially when the probability distribution of the measure of interest is poorly represented by its expected value due to heavy-tail behaviors or multiple modalities. Recent works inspired by distributional reinforcement learning use discrete histograms to approximate integer reward distribution, but they struggle with continuous reward space and present challenges in balancing accuracy and scalability. We propose a novel method for handling both continuous and discrete reward distributions in Discrete Time Markov Chains using moment matching with Erlang mixtures. By analytically deriving higher-order moments through Moment Generating Functions, our method approximates the reward distribution with theoretically bounded error while preserving the statistical properties of the true distribution. This detailed distributional insight enables the formulation and robust model checking of quality properties based on the entire reward distribution function, rather than restricting to its expected value. We include a theoretical foundation ensuring bounded approximation errors, along with an experimental evaluation demonstrating our method's accuracy and scalability in practical model-checking problems.

==> Makefile <==
# MAIN_TEX assumed as environment variable in CI/CD. If not defined, it may fall back to a hand-oded one
# to reuse the same makefile also locally.

ifeq ($(MAIN_TEX),)
MAIN_TEX := conference_101719
endif


latexcmd = pdflatex
bibcmd = bibtex
previous_commit = $(shell git log --pretty="%H" | awk "NR==2 {print $1 }")
previous_version_dir = /tmp/tmplatexdiff#$(shell mktemp -d)
latex-diff-filename = latex-diff

all: compile clean

staticchecks : compile check count clean

compile:
	# mkdir -p out
	# rm -rf _minted-main
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${MAIN_TEX}.tex 
	${bibcmd} ${MAIN_TEX}
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${MAIN_TEX}.tex 
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${MAIN_TEX}.tex 
	${bibcmd} ${MAIN_TEX}
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${MAIN_TEX}.tex 

check:
	- checkcites ${MAIN_TEX}.aux > checkcites-report.txt
	- chktex ${MAIN_TEX} > chktex-report.txt

count:
	- texcount -inc ${MAIN_TEX}.tex > texcount-report.txt

spellcheck:
	- aspell -c -t ${MAIN_TEX}.tex -d en

diff:
	cp -rT .. ${previous_version_dir}
	cd ${previous_version_dir} && git checkout ${previous_commit}
	rm -rf out
	mkdir -p out
	rm -rf _minted-main
	latexdiff --flatten ${previous_version_dir}/paper/${MAIN_TEX}.tex ${MAIN_TEX}.tex > ${latex-diff-filename}.tex
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${latex-diff-filename}.tex 
	${bibcmd} ${latex-diff-filename}
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${latex-diff-filename}.tex 
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${latex-diff-filename}.tex 
	${bibcmd} ${latex-diff-filename}
	${latexcmd} -interaction nonstopmode -halt-on-error -file-line-error --shell-escape ${latex-diff-filename}.tex 

diffclean: 
	rm -f ${latex-diff-filename}.aux
	rm -f ${latex-diff-filename}.bbl
	rm -f ${latex-diff-filename}.blg
	rm -f ${latex-diff-filename}.log
	rm -f ${latex-diff-filename}.run.xml
	rm -f ${latex-diff-filename}-blx.bib
	rm -f ${latex-diff-filename}.dvi
	rm -f ${latex-diff-filename}.ps
	rm -f ${latex-diff-filename}.pyg
	rm -f ${latex-diff-filename}.bcf
	rm -f ${latex-diff-filename}.out
	rm -rf ${latex-diff-filename}.auxlock
	rm -rf ${latex-diff-filename}.pdf_original
	rm -rf ${latex-diff-filename}.fls
	rm -rf ${latex-diff-filename}.fdb_latexmk
	rm -rf __latexindent_temp.*
	rm -rf .texpadtmp
	rm -rf _minted-main
	rm -rf *.tex~
	rm -rf sec/*.tex~
	rm -rf *.bib.blg
	rm -rf missfont.log
	rm -rf out/*.dpth
	rm -rf out/*.dep
	rm -rf out/*.log
	rm -rf out/*.run.xml

clean: 
	rm -f ${MAIN_TEX}.aux
	rm -f ${MAIN_TEX}.bbl
	rm -f ${MAIN_TEX}.blg
	rm -f ${MAIN_TEX}.log
	rm -f ${MAIN_TEX}.run.xml
	rm -f ${MAIN_TEX}-blx.bib
	rm -f ${MAIN_TEX}.dvi
	rm -f ${MAIN_TEX}.ps
	rm -f ${MAIN_TEX}.pyg
	rm -f ${MAIN_TEX}.bcf
	rm -f ${MAIN_TEX}.out
	rm -rf ${MAIN_TEX}.auxlock
	rm -rf ${MAIN_TEX}.fls
	rm -rf ${MAIN_TEX}.fdb_latexmk
	rm -rf __latexindent_temp.*
	rm -rf .texpadtmp
	rm -rf ${MAIN_TEX}.pdf_original
	rm -rf *.tex~
	rm -rf sec/*.tex~
	rm -rf *.bib.blg
	rm -rf missfont.log
	rm -rf out/*.dpth
	rm -rf out/*.dep
	rm -rf out/*.log
	rm -rf out/*.run.xml

squeaky: clean
	# rm -rf out

distclean: squeaky
	rm -rf ${MAIN_TEX}.pdf
	rm -rf ${latex-diff-filename}.pdf
	
arxiv: clean all
	arxiv_latex_cleaner .
	cd ../$(notdir $(shell pwd))_arXiv && \
		latexpand --expand-bbl ${MAIN_TEX}.bbl ${MAIN_TEX}.tex -o ${MAIN_TEX}-new.tex && \
		mv ${MAIN_TEX}-new.tex ${MAIN_TEX}.tex && \
		rm Makefile
